Hyperbolic Contrastive Learning

Learning good image representations that are beneficial to downstream tasks is a challenging task in computer vision. As such, a wide variety of self-supervised learning approaches have been proposed. Among them, contrastive learning has shown competitive performance on several benchmark datasets. The embeddings of contrastive learning are arranged on a hypersphere that results in using the inner (dot) product as a distance measurement in Euclidean space. However, the underlying structure of many scientific fields like social networks, brain imaging, and computer graphics data exhibit highly non-Euclidean latent geometry. We propose a novel contrastive learning framework to learn semantic relationships in the hyperbolic space. Hyperbolic space is a continuous version of trees that naturally owns the ability to model hierarchical structures and is thus beneficial for efficient contrastive representation learning. We also extend the proposed Hyperbolic Contrastive Learning (HCL) to the supervised domain and studied the adversarial robustness of HCL. The comprehensive experiments show that our proposed method achieves better results on self-supervised pretraining, supervised classification, and higher robust accuracy than baseline methods.

==> sections/4_ablation.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-0.8cm}
    \includegraphics[width=\linewidth]{figures/qualitative/out_of_context.pdf}
    \caption{Out-of-context images from the SUN09 dataset. The bounding box of each object and its hyperbolic distance to the scene are shown. Regular objects are in blue and out-of-context objects are in purple. Note that the out-of-context objects tend to have large distances.}
    \label{fig:oot_detection}
\end{figure*}
\section{Main Ablation Studies}
In this section, we report the results of several important ablation studies with respect to HCL. All the models are trained on the subset of the OpenImages dataset and linearly evaluated on the ImageNet-100 dataset. The top-1 accuracy is reported.


% \vspace{0.3cm}
% \centerline{\begin{minipage}{\textwidth}
% \small
% \centering
% \begin{minipage}[b]{0.363\textwidth}
% \centering
%     \begin{tabular}{ll|ll}
%     \toprule
%     Dist.  & Center & IN-100 & IPS \\
%     \midrule
%     -          & -      & 77.36   & 52.96 \\
%     \rowcolor[HTML]{DFDFDF} 
%     Hyp. & Scene  & 79.08       & 53.82 \\
%     Hyp. & Object & 76.96       & 52.74 \\
%     Euc.  & Scene  & 76.68      & 52.58 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:setup}
%   \captionof{table}{Ablation on the similarity measure and hierarchy center.}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.265\textwidth}
% \centering
%     \begin{tabular}{l|ll}
%     \toprule
%     $\lambda$ & IN-100 & IPS \\
%     \midrule
%     0.01      & 77.70        & 53.43   \\
%     \rowcolor[HTML]{DFDFDF} 
%     0.1       & 79.08        & 53.82   \\
%     0.2       & 78.64        & 53.84   \\
%     0.5       & 0            & 0       \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:lambda}
%   \captionof{table}{Ablation on the losses trade-off.}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.35\textwidth}
% \centering
%     \begin{tabular}{ll|ll}
%     \toprule
%     Optim. & $\lambda$ & IN-100 & IPS \\
%     \midrule
%     \rowcolor[HTML]{DFDFDF} 
%     RSGD & 0.1 & 79.08                      & 53.82    \\
%     RSGD & 0.5 & 0                          & 0       \\
%     SGD  & 0.1 & 70.16                      & 48.47   \\
%     SGD  & 0.5 & 74.18                      & 42.75   \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:optim}
%   \captionof{table}{Ablation on the RSGD versus SGD optimizers.}
% \end{minipage}
% \end{minipage}}
% \vspace{-0.15cm}


\begin{table*}[t]
\RawFloats
\small
\centering
\begin{minipage}[b]{0.4\textwidth}
\centering
    \begin{tabular}{llc}
    \toprule
    Distance  & Center & IN-100 Accuracy \\
    \midrule
    -          & -      & 77.36  \\
    \rowcolor[HTML]{DFDFDF} 
    Hyperbolic & Scene  & 79.08      \\
    Hyperbolic & Object & 76.96      \\
    Euclidean  & Scene  & 76.68     \\
    \bottomrule
    \end{tabular}
  \captionof{table}{Similarity measure and hierarchy center.}
    \label{tab:setup}
\end{minipage}%
\hfill
\begin{minipage}[b]{0.23\textwidth}
\centering
    \begin{tabular}{lc}
    \toprule
    $\lambda$ & IN-100 Accuracy \\
    \midrule
    0.01      & 77.70       \\
    \rowcolor[HTML]{DFDFDF} 
    0.1       & 79.08      \\
    0.2       & 78.64      \\
    0.5       & 0          \\
    \bottomrule
    \end{tabular}
  \captionof{table}{Losses trade-off.}
    \label{tab:lambda}
\end{minipage}
\hfill
\begin{minipage}[b]{0.36\textwidth}
\centering
    \begin{tabular}{llc}
    \toprule
    Optimizer & $\lambda$ & IN-100 Accuracy \\
    \midrule
    \rowcolor[HTML]{DFDFDF} 
    RSGD & 0.1 & 79.08  \\
    RSGD & 0.5 & 0      \\
    SGD  & 0.1 & 70.16  \\
    SGD  & 0.5 & 74.18  \\
    \bottomrule
    \end{tabular}
  \captionof{table}{RSGD versus SGD optimizers.}
    \label{tab:optim}
\end{minipage}
    \vspace{-0.5cm}
\end{table*}

\topic{Similarity measure and the center of the scene-object hierarchy.} We propose to use the negative hyperbolic distance as the similarity measure of the scene-object pairs. As an alternative, one can use cosine similarity on the hypersphere as the measure as in the original contrastive objective. However, this would attempt to maximize the similarity between a single object and multiple objects. It is likely that these objects belong to different classes, and hence this strategy impairs the quality of the representation. As shown in Table~\ref{tab:setup}, replacing the negative hyperbolic distance with the Euclidean similarity impairs downstream performance. The resulting model performs even worse than the baseline without loss function on the scene-object pairs, demonstrating the necessity of using hyperbolic distance. We also validate our choice of an object-centric hierarchy by comparing its performance with that of a scene-centric hierarchy~\cite{parikh2007hierarchical,parikh2009unsupervised} generated by sampling the negative pairs as objects and unpaired scenes. This scene-centric hierarchy leads to substantially lower accuracy (Table~\ref{tab:setup}). 

\topic{Trade-off between the Euclidean and hyperbolic losses.} We adopt the Euclidean loss to learn object-object similarity and the hyperbolic loss to learn object-scene similarity. A hyperparameter $\lambda$ controls the trade-off between them. As shown in Table~\ref{tab:lambda}, we find that a smaller $\lambda=0.01$ leads to marginal improvement. However, we also observe that larger $\lambda$s can lead to unstable and even stalled training. With careful inspection, we find that in the early stage of the training, the gradient provided by the hyperbolic loss can be inaccurate but strong, which pushes the representations to be close to the boundary. As a result, since Riemannian SGD divides gradients by the distance to the boundary, updates become small and training ceases to make progress.

\topic{Optimizer.} Given the observation above, we ask whether RSGD is necessary for practical usage. We replace the RSGD optimizer with SGD. To avoid numerical issues when the representations are too close to the boundary, we increase $\varepsilon$ from $1e^{-5}$ to $1e^{-1}$. This allows a larger $\lambda$ to be used as opposed to the RSGD. However, SGD always yields inferior performance compared to RSGD. %Therefore, it shows that the accurate gradient provided by RSGD is still necessary.

